zkLogin: Privacy-Preserving Blockchain Authentication with Existing Credentials

For many users, a private key based wallet serves as the primary entry point to blockchains. Commonly recommended wallet authentication methods, such as mnemonics or hardware wallets, can be cumbersome. This difficulty in user onboarding has significantly hindered the adoption of blockchain-based applications. We develop zkLogin, a novel technique that leverages identity tokens issued by popular platforms (any OpenID Connect enabled platform e.g., Google, Facebook, etc.) to authenticate transactions. At the heart of zkLogin lies a signature scheme allowing the signer to sign using their existing OpenID accounts and nothing else. This improves the user experience significantly as users do not need to remember a new secret and can reuse their existing accounts. zkLogin provides strong security and privacy guarantees. Unlike prior works, zkLogin's security relies solely on the underlying platform's authentication mechanism without the need for any additional trusted parties (e.g., trusted hardware or oracles). As the name suggests, zkLogin leverages zero-knowledge proofs (ZKP) to ensure that the sensitive link between a user's off-chain and on-chain identities is hidden, even from the platform itself. zkLogin enables a number of important applications outside blockchains. It allows billions of users to produce \textit{verifiable digital content leveraging their existing digital identities}, e.g., email address. For example, a journalist can use zkLogin to sign a news article with their email address, allowing verification of the article's authorship by any party. We have implemented and deployed zkLogin on the Sui blockchain as an additional alternative to traditional digital signature-based addresses.

==> Appendices/addr_derivation_extensions.tex <==
\section{Other Address Derivation Options}
\label{sec:addr_derivation}

We describe certain trade-offs that need to be made depending on the type of identifier used.

\paragraph{Pairwise user identifiers} One solution is to simply derive a user's address from the pairwise ID. To be more precise, the address would be $H(\sub, \iss)$ where $\iss$ is the Provider's unique identifier.

But this means that the wallet is not interoperable (property 3b) as pairwise IDs are Relying-Party specific. 
For a similar reason, this solution also implies placing significant trust (property 4) in the Relying-Party.

An attractive alternative is to decide on a set of $n$ Relying Parties (or wallet) at account creation time such that the user can login from any of the $n$ wallets.
Then, the user's address is derived as $H((\sub_1, \aud_1), \ldots, (\sub_n, \aud_n), \iss )$.
In this way, we can mitigate the problems arising from the na\"ive solution to a large extent.

\paragraph{Public user identifiers} With public IDs, the interoperability challenges go away but a new set of issues arise, as we explain now. 
A starting solution could again be to derive a user's address from the public ID, e.g., $H(\sub, \iss)$. 

But this solution has some severe issues. 
First, we create a huge account security risk (property 4) because a single malicious Relying Party can, without the knowledge of a user, include an ephemeral key into the nonce and gain the ability to sign arbitrary transactions.
Second, this solution breaks unlinkability (property 5) because $\sub$ can be highly sensitive.\footnote{Even though most of the sensitive information in a JWT is not revealed, the link between the off-chain and on-chain identities is public.}

We resolve the first challenge by binding a user address to a set of wallets (like before).
The user decides on a set of $n$ Relying Parties and the user address is $H(\sub, (\aud_1, \aud_2, \ldots, \aud_n), \iss)$.

Coming to the second issue, namely unlinkability. First note that depending on what the public ID is and the user's preferences are, the privacy risk varies. For example, users might be willing to use their Twitch subject identifier (say) as opposed to their Google subject identifier (which is more audely used). 

We propose the following approach in case unlinkability is desired.
The idea is to use an additional \textit{linking secret}~$\pin$ to provide unlinkability. 
We derive a user's address as $\userAddress = H(\sub, (\aud_1, \aud_2, \ldots, \aud_n), \iss, \pin)$.
While this solution does involve an additional secret (violating the no-secrets property), we think it is acceptable because a well-designed UX can hide the existence of this secret from the user to the extent possible.
For example, we can rely on the relying party to store the linking secret so that the user does not need to enter it in their day-to-day interaction (the user only needs this secret in the corner cases, e.g., switching devices).

% \begin{table}[]
%     \centering
%     \begin{tabular}{c|c}
%          &  \\
%          & 
%     \end{tabular}
%     \caption{Caption}
%     \label{tab:approaches}
% \end{table}

\paragraph{Note} One could argue that as defined before, the property 4 (no additional trust) is weak because the OpenID Provider is still being trusted in all the solutions. 
One reason this can be important is if the Provider suddenly decides to disallow supporting blockchain wallets.
However, this can be easily overcome by deriving the address alternatively as follows, e.g., $H((\sub_1, \aud_1, \iss_1), \ldots, (\sub_n, \aud_n, \iss_n) )$, such that the user is able to access their account as long as one of the $n$ providers are live.

% \begin{enumerate}
    % \item \textit{Trade-off unlinkability:} We can derive the user's on-chain address simply as $\userAddress = H(\sub)$, so the link between the user's OpenID identity and their blockchain address is public. Depending on what the unique ID is and the user's preferences are, the privacy risk varies. For example, users might be willing to use their Twitch subject identifier (say) as opposed to their Google subject identifier (which is more audely used for advertising and tracking purposes). 
    % Compared to prior work\deepak{cite}, we vastly minimize the amount of information revealed on-chain as all other sensitive fields in the JWT besides the key claim (e.g., name) can be hidden.
    % \item \textit{Trade-off no-trust:} In this category, we achieve unlinkability and no-secrets, but require placing some trust in the relying party for liveness, i.e., being able to access the on-chain account. The idea is to include an additional \textit{linking secret}~$\pin$ in the derivation of a user's address, i.e., we derive it as $\userAddress = H(\sub, \pin)$ where the purpose of $\pin$, as its name suggests, is just to offer unlinkability. Therefore, instead of requiring a user to remember it, we rely on the relying party to store the secret. A well-designed UX could additionally involve sending this secret to the user's email so that even if the relying party ever goes down, the user can still access the account. Note that the user is only required to enter this secret when they are switching wallets, so .
% \end{enumerate}

% That is, this secret is backed-up by the relying party on behalf of the user. Note that the only time a user needs to be aware of the existence of a PIN is when switching wallets, which is a slight deviation from the no-secrets goal. 
    % Yet again, a crucial distinction from prior work \deepak{cite} is that they require placing extra trust for account safety, \textit{which we do not}. 


==> extensions.tex <==
\section{Extensions}
\label{sec:extensions}

\begin{itemize}
    \item Multi-sigs
    \item  Custody-less property
    \item  2-of-3
    \item  Groth vs. PLONK
    \item  Can we simulate in PLONK with just KZG toxic waste?
    \item  non-repudiation with transparent
    \item  Threshold zkCookie, Threshold signing
    \item  Paragraph where self-setup and toxic waste are useful/harmless
    \item Enlist applications, creating a CA, DV-NIZK, Owned L2 (self-audit), Authentication, Group/Ring signatures
    \item spell out witness hiding property
    \item  Leveraging OpenPubKey to bind Web2 id to zkcrs
    \item  Toxic waste vs revealing proving key
    \item  Universal circuit vs specific circuits
    \item  Hide logic in private circuit
    \item  Private vs stateless-ness tradeoffs
\end{itemize}

\subsection{MultiSig to Threshold Compiler}


==> tasks.tex <==
\section*{To Do}

\begin{enumerate}
    \item Review requests:
    \begin{itemize}
        \item Abstract: Kostas
        \item Introduction: Foteini
        \item Preliminaries: Mahdi
        \item Tagged Witness Signature: Mahdi
        \item The zkLogin System: Kostas
        \item Implementation and Evaluation: Ben/Kostas, Jonas, Joy
        \item Related Works: Ben, Foteini
    \end{itemize}
\end{enumerate}



% \begin{enumerate}
%     \item Discussion of why ceremony was needed, especially in contrast to self-generation
%     \item Streamline formatting. $\lambda \rightarrow 1^{\lambda}$ everywhere
%     \item Refer to the privacy property captured by \TWS. Pass on Section 3.1 to reconcile \TWS with informal properties.
%     \item Recast extractor in \TWS as an indist game
%     \item Define EUF-CMA for signatures. How JWT.Issue captures this.
%     \item Capture $\expiryTime \geq \curTime$ in the proof.
%     \item (Done) Use the APIs in Section 2.1 in the proof.
%     \item Work on the table in terms of various protocol modes with properties: unforgeability, privacy, discoverability.
% \end{enumerate}

% \begin{enumerate}
%     \item [AR] Witness Signature: formal description and security proofs
%     \item [DM] Proof structure of OpenID-ZKP-Auth
%     \item [MS] 1) Relation of WS and Signatures of knowledge 2) Extensions: vk Equivocation
%     \item proposal for how to present our constructions:
%     \begin{enumerate}
%         \item talk about the reqs: preventing replay attacks, compromised wallet backend, compromised wallet (which should be solved using other methods), phishing attacks (other oauth providers)

%         then present how to build a solution...
        
%         \item pubopenid (or actually the gnosis solution from 2019) as is - not private (say why: jwts usually has sensitive fields, or not everyone use pairwise ids and then it's easy to find who is the user)
%         \item for solving privacy, one could do everything inside zk -> that won't be very efficient, and we can do better by splitting the verification to (1) sig verification, (2) jwt verification
%         \item openid (with standard nonce) + zk on [jwt | ephemeral pk] + sig verify - this one is indeed private, however the wallet backend (which sees the jwt token) can impersonate onchain as the user
%         \item pubopenid with special nonce + zk on jwt + sig verify - private because of the zk, safe against compromised wallet backend because of the nonce trick
%         \item then we can have a section about efficient zk, including using groth16 without a trusted setup (benefits...), highly tailored boolean circuit, etc
%         \item section about how to retrieve the id providers' public keys (DAO managed, fetched by nodes, etc)
%     \end{enumerate}
% \end{enumerate}


